Parameter estimation from the core-bounce phase of rotating core collapse supernovae in real interferometer noise

In this work we propose an analytical model that reproduces the core-bounds phase of gravitational waves (GW) of Rapidly Rotating (RR) from Core Collapse Supernovae (CCSNe), as a function of three parameters, the arrival time $\tau$, the ratio of the kinetic and potential energy $\beta$ and a phenomenological parameter $\alpha$ related to rotation and equation of state (EOS). To validate the model we use 126 waveforms from the Richers catalog \cite{Richers_2017} selected with the criteria of exploring a range of rotation profiles, and involving EOS. To quantify the degree of accuracy of the proposed model, with a particular focus on the rotation parameter $\beta$, we show that the average Fitting Factor (FF) between the simulated waveforms with the templates is 94.4\%. In order to estimate the parameters we propose a frequentist matched filtering approach in real interferometric noise which does not require assigning any priors. We use the Matched Filter (MF) technique, where we inject a bank of templates considering simulated colored Gaussian noise and the real noise of O3L1. For example for A300w6.00\_BHBLP at 10Kpc we obtain a standar deviation of $\sigma = 3.34\times 10^{-3}$ for simulated colored Gaussian noise and $\sigma= 1.46\times 10^{-2}$ for real noise. On the other hand, from the asymptotic expansion of the variance we obtain the theoretical minimum error for $\hat{\beta}$ at 10 kpc and optimal orientation. The estimation error in this case is from $10^{-2}$ to $10^{-3}$ as $\beta$ increases. We show that the results of the estimation error of $\beta$ for the 3-parameter space (3D) is consistent with the single-parameter space (1D), which allows us to conclude that $\beta$ is decoupled from the others two parameters.

==> macros.tex <==
% macros.tex
%
% LaTeX macros for S5 1st year all-sky burst search paper

% $Id: macros.tex,v 1.3 2013/12/29 17:41:00 cott Exp $

% macro for 
\newcommand\note[1]{\textcolor{red}{\bf {#1}}}

%% Today macro \today
\renewcommand{\today}{\number\day\space\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\year}
\newcommand\checkme[1]{\textcolor{blue}{#1}}

\def\etc{{\it etc.}}
\def\eg{{\it e.g.}}
\def\vs{{\it vs.}}
\def\etal{{\it et al.}}
\def\ie{{\it i.e.}}
\def\cf{{\it cf.}}
\def\mycaps#1{{\textsc{\small #1}}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}} 
\def\ei{\end{itemize}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
%%\def\i{\item{}}      %--  \i is used to produce a dotless i, needed for Diaz
%\def\hrssu{\mathrm{strain}/\sqrt{\mathrm{Hz}}}
%\def\hrssu{strain/\sqrt{Hz}}
\def\hrssu{Hz${}^{-1/2}$}
\def\hrss{h_\mathrm{rss}}
\def\hrssfifty{h_\mathrm{rss}^\mathrm{50\%}}
\def\hdet{h_\mathrm{det}}
\def\rninety{R_\mathrm{90\%}}
\def\Zcoh{Z_{\text{H}_+}}
\def\Zcor{Z^{corr}_{\text{H}_+}}
\def\sfyo{S5y1}
\def\sfyt{S5y2}
\def\ligodoc{{LIGO-P17}{00177}{}} % leave in the extra {}s -- trust me

\def\aj{Astron. J.}
\def\apj{Astrophys. J.}
\def\apjl{Astrophys. J. Lett.}
\def\apjs{Astrophys. J. Supp. Ser. }
\def\aa{Astron. Astrophys. }
\def\aap{Astron. Astrophys. }
\def\araa{Ann.\ Rev. Astron. Astroph. }
\def\aapr{Astron. Astrophys. Rev. }
\def\physrep{Phys. Rep. }
\def\mnras{Mon. Not. Roy. Astron. Soc. }
\def\mmsun{M_\odot}
\def\prl{Phys. Rev. Lett.}
\def\prd{Phys. Rev. D.}
\def\azh{Soviet Astron.}
\def\apss{Astrophys. Space Sci.}
\def\cqg{Class. Quantum Grav.}
\def\memsai{Mem. Societa Astronomica Italiana}

